Ranking Papers by their Short-Term Scientific Impact

The constantly increasing rate at which scientific papers are published makes it difficult for researchers to identify papers that currently impact the research field of their interest. Hence, approaches to effectively identify papers of high impact have attracted great attention in the past. In this work, we present a method that seeks to rank papers based on their estimated short-term impact, as measured by the number of citations received in the near future. Similar to previous work, our method models a researcher as she explores the paper citation network. The key aspect is that we incorporate an attention-based mechanism, akin to a time-restricted version of preferential attachment, to explicitly capture a researcher's preference to read papers which received a lot of attention recently. A detailed experimental evaluation on four real citation datasets across disciplines, shows that our approach is more effective than previous work in ranking papers based on their short-term impact.

==> method.tex <==
\section{Our Approach}
\label{sec-method}



The main hypothesis of our work is that researchers tend to read and cite trending papers, %that are trending, 
i.e., papers that have recently received significant attention 
from the scientific community.
To investigate
this hypothesis, we explore 
four citation networks (as per the default experimental configuration discussed in Section~\ref{sec:exp:methodology}), and count how many top-$100$ papers %, according to 
%short-term impact,
%STI, 
were recently popular, based on STI
(i.e., were among the top cited 
%papers 
in the past $5$ years). 
%has been top in receiving citations in the last $5$ years). 
%Specifically,
As we see in Table~\ref{tab:attention}, % that %approximately 
roughly half of the top-$100$ papers were, indeed, recently popular.

\iffalse
\begin{table}[t]
\centering
\caption{Recently popular papers in top-$100$ (accord. to STI)}
\label{tab:attention}
\begin{tabular}{c|c}
\hline
\textbf{Dataset} & \textbf{Recently popular}  \\
\hline
hep-th   & $41$ \\
APS & $54$\\
PMC & $54$ \\
DBLP & $63$ \\
\hline
\end{tabular}
\end{table}
\fi

\begin{table}[t]
\centering
\caption{Recently popular papers in top-$100$ (accord. to STI)}
\label{tab:attention}
\begin{tabular}{c|c c c c}
\hline
\textbf{Dataset} & \textbf{hep-th} & \textbf{APS} &
\textbf{PMC} & \textbf{DBLP} \\
\hline
\textbf{Recently Popular} & $41$ & $54$ & $54$ & $63$\\
\hline
\end{tabular}

\end{table}


This observation validates our assumption that the level of attention a paper has recently attracted is indicative of its ability to attract citations in the short-term.
% \footnote{{\color{cyan}In this 
% work we do not discern among different citation
% profiles as in~\cite{chakraborty2015categorization}.
% Instead, we use recent citation data as an 
% indicator of the situation in the short-term,
% in a generalised manner.}}
We thus propose the following method to quantify recent attention. Let $\mathbf{C}[t_N\!-\!y \!:\! t_N]$ denote
the citation matrix
taking into account only citations
made during the past $y$ years.
The recent attention, simply called \emph{attention}, of a paper $ p_i $ is calculated as:
%
\begin{equation}
\label{prefat}
    A(p_i) = \frac{\sum_j{C[t_N\!-\!y \!:\! t_N][i,j]}}{\sum_i{\sum_j{C[t_N\!-\!y \!:\! t_N][i,j]}}},
\end{equation}
%
which corresponds to the 
fraction of total citations in the last $y$ years, which %that were made to 
paper $p_i$ received. Hyperparameter $y$ induces time-awareness, allowing us to capture the most recent dynamics; its value is to be tuned for the specific ranking problem.



Attention, however, is not the only mechanism that governs which papers researchers read. Naturally, researchers may read a paper cited in the reference list of another paper. Moreover, similar to previous work \cite{walker2007ranking,sayyadi2009futurerank}, we assume that researchers also read recently published papers. Specifically, we capture the recency of a paper $p_i$ using a score that decays exponentially based on the paper's age:
%
\begin{equation}
\label{exponential-factor}
    T(p_i) = c \cdot e^{w \cdot (t_N - t_{p_i})},
\end{equation}
%
where $ t_N $ is the current time,
$ t_{p_i} $ denotes the publication time 
of paper $ p_i $, hyperparameter $ w $ is 
a negative constant (as $t_N-t_{p_i}\geq 0$),
and $c$ is normalization constant so that $\sum_i T(p_i)=1$.
To calculate a proper $w$ value, a similar 
procedure like the one used in~\cite{sayyadi2009futurerank} can be 
followed (see also Section~\ref{param_tuning}).


Combining these mechanisms, we assume that
a researcher may read %cite 
a paper for one of 
the following reasons: the paper gathered 
attention recently, the paper was recently published, 
or the paper was found in another paper's
reference list. We model this behavior with the following random process.
% in a 
% PageRank-like random walk process, with
% a probability value corresponding to each
% of these ways in which researchers
% choose to read a paper. In particular, \sout{We are now ready to describe the complete model of a researcher's selection process of papers to read.} 
% \sout{T}t}he
A researcher, after %upon finishing 
reading paper 
$ p_i$, chooses to read any other paper from $ p_i $'s 
reference list, with probability $ \alpha $. %Moreover, with
With probability $ \beta $ she 
chooses a paper
based on its attention. 
This behavior essentially makes recently rich papers even richer, and is reminiscent of a 
time-restricted preferential attachment mechanism 
%in the Barab\'asi-Albert model of network growth
of the Barab\'asi-Albert model of network
growth~\cite{barabasi2014network}.
%restricted in a small time frame.
Finally, with probability $ \gamma $
she chooses 
any paper with a
preference towards recently published ones. 


Specifically, our model computes a score $AR(p_i)$, called \method, for each paper $p_i$ that satisfies the following recurrence:
%
\begin{equation}
\label{PAPER:equation} 
AR(p_i)  = \alpha \cdot \left(\sum_j{ S[i,j] \cdot AR(p_j)}\right) + \beta \cdot A(p_i) + \gamma \cdot T(p_i),
\end{equation}
%
where the coefficients $ \alpha, \beta, \gamma \in [0,1] $
and $ \alpha + \beta + \gamma = 1 $, and
$ \mathbf{S} $ is the stochastic 
citation matrix as defined in PageRank. As is typical, the optimal values for the three coefficients are to be determined by validation. 

Two special values for coefficient $\beta$ are worth mentioning.
First, observe that when $\beta=0$, a setting we call NO-ATT (for no attention), the model becomes similar to time-aware methods that address the inherent bias against new papers in citation networks (see also Section~\ref{sec-related}, and \cite{KVSDV2019} for a thorough coverage of such approaches). Note that additionally setting $w=0$ in Eq.~\ref{exponential-factor} recovers PageRank. Second, when $\beta=1$, a setting we call ATT-ONLY (for attention only), \method is solely based on the attention mechanism, assuming that the recent citation patterns will persist exactly in the near future. To the best of our knowledge, ATT-ONLY has not been considered in the literature as a means to estimate the short-term impact of a paper. As we %investigate
show in Section~\ref{sec-exp}, attention alone is a powerful mechanism, %that is 
often more effective than existing approaches. However, $\beta=1$ is never the optimal setting; it is always better to consider attention in combination with the other two citation mechanisms.


% \mnote[TV]{Maybe discuss here that the attention is an important parameter as shown both by Table~\ref{tab:attention} and by our experiments ... if you see that when $\beta$ is near zero then ... }

\iffalse
\stitle{Citation Network growth Model.}
%
Citation networks fall under the so-called 
category of \emph{fat tailed}
networks~\cite{barabasi2014network}
This means that they are composed mainly
of papers that have a small 
in-degree (citation count), with the
additional existence of \emph{hubs}, papers
that have an in-degree that is orders of magnitude 
higher than that of most nodes. Fat-tailed
networks are best approximated as scale 
free networks, i.e., networks for which the
distribution of node degrees follows a
\emph{power law}\footnote{This means that
the distribution of the degree of nodes
follows: 
$ p(k) \thicksim k^{-\gamma} $, where $ k $ 
is a node's degree, $ p(k) $ is the
probability of the node having degree 
equal to $ k $, and $ \gamma $ is a positive 
number.}~\cite{barabasi2014network}.


Barab\'asi and Albert introduced a minimal model 
that captures the two mechanisms 
responsible for the emergence of 
the aforementioned degree
distribution in networks \cite{barabasi2014network}:
\emph{growth}: the network
is not static, but expands with the addition of new nodes;
and \emph{preferential attachment}: each newly added
node connects to any of the
previously added ones with
probability proportional to their degrees.


We propose a time-aware variant of the aforementioned mechanisms, better suited for citation networks. The intuition is that the network growth is driven by the recent popularity of papers. 
\fi





\iffalse
equal to the fraction
of total edges in the network they have.

The preferential attachment probability
is defined as follows:

\begin{equation}
\label{preferential-attachment}
\Pi(n_i) = \frac{d_{n_i}}{\sum_{j}{d_{n_j}}}
\end{equation}

In Equation~\ref{preferential-attachment},
$ d_{n_i} $ denotes the degree of node 
$ {n_i} $. 
Equation~\ref{preferential-attachment} states
that a new node added to the network
is more likely to connect to those nodes 
that already have a high degree, with
probability equal to their fraction of total
edges in the network.

Note, that the aforementioned model cannot
explain all growth phenomena of real networks,
e.g., how new nodes can acquire a large 
number of links (e.g., links to web-sites 
such as Facebook, which arrived late on the
WWW, or citations to breakthrough papers in
citation networks). This would require 
incorporating additional, more complex
mechanisms related to each particular 
network type~\cite{barabasi2014network}.
\mnote[IK]{Maybe add here that the model
is introduced to explain mechanisms that
lead to long tail distributions. It doesn't
necessarily attempt to describe all network
processes, hence doesn't capture thing like
papers that \emph{start} being cited while
initially they are at 0, or papers that 
\emph{stop} being cited although they 
should have a high preferential attachment
probability. I'm not sure we make this clear
enough in the previous passage. On the other
hand I am not 100\% sure if we have to... ideas?}

\fi


\iffalse

PageRank-based methods that have been 
proposed to rank papers, typically simulate
researchers who read a paper and then either
proceed to read one of the papers in its
reference list, or choose any paper to read 
at random. Particularly, to tackle citation
lag, the simulated researchers are modelled 
to prefer either a) to choose recently
published papers when following references
(e.g.,
in~\cite{walker2007ranking,yu2004temporal}),
b) to prefer recently published papers when
randomly choosing one to read
(e.g. in~\cite{sayyadi2009futurerank}), 
or c) to choose recently  published papers
when making either of the previous two 
choices
%, i.e., either when following references,
%or when choosing any paper 
(e.g., in~\cite{hwang2010yet,dunaiski2012comparing}).
Each method, thus, calculates scores that
reflect how ``easily" papers are found by a
researcher, under the modelled behaviour. 
However, in our view, researchers do
not only cite papers by finding them
through references, or by selecting
recent papers.\mnote[IK]{maybe change this. 
there were comments about the ``citing" part. 
We could rewrite this to say not that the researchers
cite, but that they start reading papers that gather 
attention at random walk restarts} Particularly, researchers 
also directly cite currently well-cited 
papers (regardless of their age), 
reflecting their work on current research
trends or on furthering previous research. 
To capture this additional behaviour, 
we modify PageRank's model, incorporating
mechanisms from the network growth model
proposed by Barab\'asi and  Albert 
(see Section~\ref{network-growth}). 

{\color{red}Our method, %PA-Rank,
\method~(AR), is based on PageRank 
with a modification on its random jump vector.
Particularly, we use two vectors, 
in place of PageRank's uniformly distributed
random jump vector: one based on weights 
that decrease exponentially based on paper
age, and a new, second vector calculated 
based on a preferential attachment score 
for each paper, {\color{blue}based on} a 
recent time period. \mnote[IK]{TOO MANY BASED ON'S!! 
REWRITE}}
\iffalse 
Thus, in our model, we retain the 
behaviour of a researcher following
references with equal probability,
when choosing to read a paper from a 
reference list, as is the case in PageRank.
Additionally we model the behaviour of
a researcher choosing to read papers in 
the citation network with a preference 
towards recently published ones when not
following references (this type of weight 
has also been used by 
other methods, such
as~\cite{walker2007ranking,sayyadi2009futurerank}). 
However, we add a further
random jump to the researcher's behaviour,
which is based on a preferential
attachment probability for each paper (see
Section~\ref{network-growth}). 
\fi 
Our model is formally described as follows:

\begin{equation}
\label{PAPER:equation} 
AR(p_i)  = \alpha \cdot \left(\sum_j{ S[i,j] \cdot AR(p_j)}\right) + \beta \cdot A(p_i) + \gamma \cdot T(p_i) 
\end{equation}

In Equation~\ref{PAPER:equation},
$ AR(p_i) $  is the %PA-Rank  
\method~score 
of paper $ p_i $, the 
coefficients $ \alpha, \beta, \gamma \in [0,1] $
and $ \alpha + \beta + \gamma = 1 $.
%and  $ \alpha, \beta, \gamma \neq 0 $. 
$ \mathbf{S} $ is the same stochastic 
citation matrix used in PageRank. 
$ \mathbf{T} $ is an exponential 
``random" jump probability (this type of 
weight has also been used
in~\cite{walker2007ranking,sayyadi2009futurerank}), 
normalized for all papers so that their 
$ T(p_i) $ scores have a sum equal to~1. 
It is calculated as:

\begin{equation}
\label{exponential-factor}
    T(p_i) = e^{w * (t_N - t_{p_i})}
\end{equation}

In Equation~\ref{exponential-factor}, 
$ t_N $ denotes the current year, while 
$ t_{p_i} $ denotes the publication year 
of paper $ p_i $. Parameter $ w $, is 
a negative constant ($t_N-t_{p_i}\geq 0$). 
To calculate a proper $w$ value, a similar 
procedure like the one used in~\cite{sayyadi2009futurerank} can be 
followed (see also Section~\ref{param_tuning}). 
%We calculate $ w $ 
%as follows: for a collection of papers we 
%take the best exponential fit for the 
%average number of citations that papers 
%in this collection receive $ n $ years 
%after their publication. This is the 
%same procedure used
%in~\cite{sayyadi2009futurerank}.
%\mnote[IK]{We repeat this idea later in 
%Section 4.4. Should we remove it from
%one of the two sections?}

$ \mathbf{A} $ is a preferential
attachment probability for each paper 
$ p_i $, calculated in a recent time 
period, as follows: 

\begin{equation}
\label{prefat}
    A(p_i) = \frac{\sum_{j=1}^{|P|}{C^{y}[i,j]}}{\sum_{i=1}^{|P|}{\sum_{j=1}^{|P|}{C^{y}[i,j]}}}
\end{equation}

In Equation~\ref{prefat}, $ C^{y} $ is 
a citation matrix of the citation network,
which takes into account only those citations
made during the last $y$ years. Thus, 
$ C^y[i,j] = 1 $ iff paper $ p_j $ cites
paper $p_i $ in the last $y$ years, 
or $ C[i,j] = 0 $ otherwise.
In other words, $ A(p_i)  $ is a
probability, which corresponds to the 
fraction of total references in the citation
network, that were made to paper $ p_i $
in the last $y$ years. We use only a recent
time frame, rather than all of the dataset's
time span, to capture the most recent network
growth dynamics.

Taking the above into account, our model
simulates the behaviour of a researcher who
acts as follows: he starts reading a paper 
$ p_i$ and with probability $ \alpha $ 
chooses any other paper from $ p_i $'s 
reference list to read, similarly to simple
PageRank. With probability $ \gamma $
he chooses 
any paper in the citation network, with a
preference towards recently published ones,
similarly to~\cite{walker2007ranking,sayyadi2009futurerank}. 
Finally, with probability $ \beta $ he 
chooses any paper in the citation network,
based on how many citations it gathered 
from year $ y $ onward. This latter behaviour
``forces" the modelled researcher to prefer
reading papers he is {\color{red}more likely to cite}
(e.g., because they deal with currently
prominent research fields), based on the
preferential attachment probability of the
Barab\'asi-Albert network growth model, 
calculated in a recent, small time frame.
\fi


\iffalse 
``corrects" the bias
of other PageRank-based methods in favor of 
simply recently \emph{published} papers,
favoring instead recently \emph{cited} ones, 
regardless of age.
\fi 
\iffalse 
Further, taking into account
the network growth mechanisms presented in
Section~\ref{}, it is a more suitable method to
predict which papers are more likely to be cited in 
the following years.
\fi


Equation~\ref{PAPER:equation} describes an iterative process for computing the $AR$ vector: starting with a random value, at each step update the vector with the right hand side of Eq.~\ref{PAPER:equation}. This process is repeated until the $AR$ values converge. The following theorem, ensures that convergence is achievable.
 
\begin{theorem}
\label{th:convergence}
The iterative process defined by Eq.~\ref{PAPER:equation} converges.
\end{theorem}

\begin{proof}



\iffalse 
$ PAPER $ is guaranteed to converge
based on the following: 
\fi 
We can rewrite 
Equation~\ref{prefat} in matrix form as:
%
\begin{equation}
\label{paper:vector}
AR = \mathbf{R}\, AR
\end{equation}
%
where $\mathbf{R}$ is a matrix satisfying:

\begin{equation}
    \label{matrix:R}
    %\begin{split}
    R[i,j]  = \alpha \cdot S[i,j] %\\
    + \beta \cdot A(p_i) %\\
    + \gamma \cdot T(p_i)
    %\end{split}
\end{equation}

In other words, matrix $ \mathbf{R} $ is a modified
citation matrix, artificially expanded with
directed edges from any node to any other in the
network. For each column $c$ of matrix $ \mathbf{R} $,
the following property holds:
%
\begin{equation}
    \label{column:sum}
    \begin{split}
    \sum_i {R[i,c]} & = 
    \alpha \cdot \sum_i {S[i,c]}
    + \beta \cdot \sum_i{A(p_i)}
    + \gamma \cdot \sum_i{T(p_i)}\\ 
     & = \alpha + \beta + \gamma = 1
    \end{split}
\end{equation}
%
Equation~\ref{column:sum} holds, because
(a) the sum over all $A$ scores 
equals 1, since these scores are probabilities,
(b) by definition the sum over all $T$ scores,
equals 1,
%, as well,  (normalized scores)}
%since we normalize these scores 
and (c) $ \mathbf{S} $ is a column
stochastic matrix, thus by definition each of
its columns has values that sum up to 1.
Hence, matrix
$ \mathbf{R} $ is also a stochastic matrix and
Equation~\ref{paper:vector} represents a power method
equation applied on matrix $ \mathbf{R} $. 

The power method on a stochastic matrix
converges, under the following
conditions~\cite{langville2011google}: 
matrix $ \mathbf{R} $ must be irreducible
and aperiodic. Irreducibility is guaranteed
for any matrix that corresponds to a strongly
connected graph, while aperiodicity is
guaranteed if $ R[i,i] > 0 $. Both 
conditions hold for matrix $ \mathbf{R} $,
due to the fact that we added artificial 
edges connecting each node to any other 
node in the citation network, as well as
itself.\footnote{Since the time-based vector
is exponentially decreasing based on paper
age, $ T(p_i) > 0, \forall p_i $. Thus,
in matrix $ \mathbf{R} $ there is a link
(however low-weight) from all nodes to 
all others.} Therefore, the iterative process is
guaranteed to converge to a single vector of 
\method~scores. \qed
%
\end{proof}

